Transportation Modes Classification Using Feature Engineering

Predicting transportation modes from GPS (Global Positioning System) records is a hot topic in the trajectory mining domain. Each GPS record is called a trajectory point and a trajectory is a sequence of these points. Trajectory mining has applications including but not limited to transportation mode detection, tourism, traffic congestion, smart cities management, animal behaviour analysis, environmental preservation, and traffic dynamics are some of the trajectory mining applications. Transportation modes prediction as one of the tasks in human mobility and vehicle mobility applications plays an important role in resource allocation, traffic management systems, tourism planning and accident detection. In this work, the proposed framework in Etemad et al. is extended to consider other aspects in the task of transportation modes prediction. Wrapper search and information retrieval methods were investigated to find the best subset of trajectory features. Finding the best classifier and the best feature subset, the framework is compared against two related papers that applied deep learning methods. The results show that our framework achieved better performance. Moreover, the ground truth noise removal improved accuracy of transportation modes prediction task; however, the assumption of having access to test set labels in pre-processing task is invalid. Furthermore, the cross validation approaches were investigated and the performance results show that the random cross validation method provides optimistic results.

==> chapters/deletedparts.tex <==

\section{Features analysis}


In order to evaluate the effect of the proposed features, the following experiments were conducted. 
A random forest classifier with 50 estimator was selected to apply in all the following test. A five-fold cross validation using the user oriented method, similar to Endo et al. (2016) \cite{endo2016deep}, was applied to measure the accuracy in each test.
The first experiment goal is to find is there a significant difference between using proposed point features.
First, the point features were grouped into different sets including [speed], [speed, acceleration], [speed, acceleration, bearing], [speed, acceleration, bearing, bearing, jerk], [speed, acceleration, bearing, jerk], [speed, acceleration, bearing, jerk, bearing-rate], and [speed, acceleration, bearing, jerk, bearing-rate, rate-of-bearing-rate] called set A, B, C, D, E, F respectively. 
We select speed point feature as minimum set and add one point feature in each iteration to see the difference between the point feature added.
The normality of cross validation results were tested using The Shapiro test and the Kolmogorov-Smirnov test for goodness of fit. Table \ref{table:shapiro1} shows the results for the Shapiro test that all the p-values are greater than 0.05 which means the null hypothesis can not be rejected. The Kolmogorov-Smirnov test shows we must reject the null hypothesis;
suggesting the data does not come from a normal distribution.
Thus, the non-parametric the Wilcoxon rank-sum statistic for two samples was chosen to compare the distribution of the observations. The null hypothesis of this test suggests that "two sets of measurements are drawn from the same distribution"\cite{scikit-learn}. Since the P-value is greater than 0.05, The null hypothesis can not be rejected. Hence, we do not have evidence to claim adding feature points to speed makes significant difference in accuracy of classifier.
%Checked OK

\begin{table}[ht]
\centering
\caption{Shapiro test results for checking the normality of cross validation results. }
\label{table:shapiro1}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E} & \textbf{F} \\ \hline
\textbf{ statistic} &  0.885150 &  0.907161 &  0.956038 &  0.769676 &  0.876981 &  0.804931 \\ \hline
\textbf{ p-value}   &  0.333303 &  0.450719 &  0.780164 &  0.044822 &  0.295855 &  0.088836 \\ \hline
\end{tabular}
\end{table}

%\textcolor{red}{What model you used to calculate accuracy?}
Figure \ref{fig:catset} shows the accuracy result of five fold cross validation for all the sets.

\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for different trajectory feature sets}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/catSet.png}
%\vspace*{1.5in}
\label{fig:catset}
\end{figure}

A same experiment with same settings was performed for trajectory features for each point feature. 
Figure \ref{fig:speedSet} shows the five fold cross validation results which depicts the importance of trajectory features of speed.  

\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for trajectory features of speed}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/speedSet.png}
\label{fig:speedSet}
\end{figure}

The shapiro test, shown in table \ref{tab:shapiro2}, and the Kolmogorov-Smirnov test were conducted to check the normality of cross validation results for trajectory features of speed. 
The results shows that we need to use non-parametric testbecause the distribution of observation does not come from normal distribution.
The non-parametric Kruskal-Wallis test was chosen to compare the median of all trajectory features for speed.

\begin{table}[]
\centering
\caption{Shapiro test results for checking the normality of trajectory features of speed}
\label{tab:shapiro2}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
\textbf{ statistic} &  0.92 &  0.97 &  0.81 &  0.96 &  0.89 &  0.95 &  0.83 &  0.96 &  0.85 &  0.89 \\ \hline
\textbf{ p-value}   &  0.56 &  0.92 &  0.10 &  0.82 &  0.38 &  0.73 &  0.14 &  0.82 &  0.22 &  0.37 \\ \hline
\end{tabular}
\end{table}
%  Kruskal-Wallis test the null hypothesis that the population median of all of the groups are equal.
The results of Kruskal-Wallis test suggests that there is statistically significant difference between accuracy score of different trajectory features of speed ($H(9)=34.967,p-value=6.0376 e-05$) with a mean rank of 0.4603 for speed mean, 0.3115 for speed max, 0.2475 for speed mean, 0.4915 for speed median, 0.3042 for speed std, 0.3308 for speed percentile 10, 0.4336 for speed percentile 25, 0.4915 for speed percentile 50, 0.5719 for speed percentile 75, and 0.6094 for speed percentile 90.

Table \ref{tab:Wilcoxon1} shows the p-values of the Kruskal-Wallis test for pairwise trajectory features of speed. 
These results most of the trajectory features of speed account for classification performance. The numbers more than 0.05 in this table means there is no significant difference between two variables in accuracy of classification. Moreover, it shows that median and percentile 50 behave in a same way and one of them can be removed. Figure \ref{fig:accSet},\ref{fig:jerkSet},\ref{fig:bearingSet},\ref{fig:brateSet} and \ref{fig:brate2Set} show the accuracy of five fold cross validation for point features including acceleration, jerk, bearing, bearing rate, and the rate of the bearing rate, respectively. 


\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for trajectory features of acceleration}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/accSet.png}
\label{fig:accSet}
\end{figure}



\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for trajectory features of jerk}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/jerkSet.png}
\label{fig:jerkSet}
\end{figure}


\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for trajectory features of bearing}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/bearingSet.png}
\label{fig:bearingSet}
\end{figure}


\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for trajectory features of bearing rate}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/brateSet.png}
\label{fig:brateSet}
\end{figure}



\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for trajectory features of the rate of the bearing rate}
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/brate2Set.png}
\label{fig:brate2Set}
\end{figure}

According to Table \ref{tab:acc}, \ref{tab:jerk}, \ref{tab:bearing}, \ref{tab:brate}, and \ref{tab:brate2} there is no statistically significant difference between all the features except bearing rate min. 
Moreover, speed percentile 50 and speed minimum are not significantly different than speed median. Therefore, the [speed max, speed mean, speed median, speed std, speed p10, speed p25, speed p75, speed p90, bearing rate min] is selected as a new trajectory feature set called \textit{Selected Features}. The \textit{Full Features} is the set of all trajectory features of speed, acceleration, jerk, bearing, bearing rate, and the rate of the bearing rate.
An experiment is conducted to investigate Is there a significant difference between using \textit{Full Features} and \textit{Selected Features}. 
Figure \ref{fig:newSet} shows the results of five fold cross validation for \textit{Full Features} and \textit{Selected Features}. 

The non-parametric Wilcoxon rank-sum statistic for two samples was chosen to compare the distribution of five fold cross validation accuracy for \textit{Full Features} and \textit{Selected Features}.
%#H0: the null hypothesis that two sets of measurements are drawn from the same distribution. 
%#The alternative hypothesis is that values in one sample are more likely to be larger than the values in the other sample.

The results of the test suggests that the null hypothesis can not be rejected. There was no statistically significant difference between accuracy score of \textit{Full Features} and \textit{Selected Features} (p-value=0.9168) with a mean of 0.6884 for \textit{Full Features}, 0.6937 for set \textit{Selected Features}. 
Therefore, the \textit{Selected Features} are the most important trajectory features and we can say  $Speed$ is the latent variable in transportation mode prediction task.


\begin{figure}[ht]
\caption{Comparing the results of 5 fold cross validation for  $Full Features$ and $Selected Features$ }
\centering
\includegraphics[width=0.8\textwidth]{chapters/fig/newSet.png}
\label{fig:newSet}
\end{figure}



\subsection{First appendix}
\begin{table}[h]
\centering
\caption{The Kruskal-Wallis test results for pair-wise trajectory features of speed. }

\label{tab:Wilcoxon1}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
min    &  1.00 &  0.12 &  0.05 &    0.92 &  0.17 &  0.25 &  0.60 &  0.92 &  0.46 &  0.12 \\\hline
max    &  0.12 &  1.00 &  0.12 &    0.01 &  0.75 &  0.75 &  0.01 &  0.01 &  0.01 &  0.01 \\\hline
mean   &  0.05 &  0.12 &  1.00 &    0.01 &  0.17 &  0.08 &  0.01 &  0.01 &  0.01 &  0.01 \\\hline
median &  0.92 &  0.01 &  0.01 &    1.00 &  0.01 &  0.02 &  0.17 &  1.00 &  0.12 &  0.08 \\\hline
std    &  0.17 &  0.75 &  0.17 &    0.01 &  1.00 &  0.46 &  0.02 &  0.01 &  0.01 &  0.01 \\\hline
p10    &  0.25 &  0.75 &  0.08 &    0.02 &  0.46 &  1.00 &  0.03 &  0.02 &  0.01 &  0.01 \\\hline
p25    &  0.60 &  0.01 &  0.01 &    0.17 &  0.02 &  0.03 &  1.00 &  0.17 &  0.03 &  0.02 \\\hline
p50    &  0.92 &  0.01 &  0.01 &    1.00 &  0.01 &  0.02 &  0.17 &  1.00 &  0.12 &  0.08 \\\hline
p75    &  0.46 &  0.01 &  0.01 &    0.12 &  0.01 &  0.01 &  0.03 &  0.12 &  1.00 &  0.35 \\\hline
p90    &  0.12 &  0.01 &  0.01 &    0.08 &  0.01 &  0.01 &  0.02 &  0.08 &  0.35 &  1.00 \\\hline
\end{tabular}
\end{table}




\begin{table}[h]
\centering
\caption{The Kruskal-Wallis test results for pair-wise trajectory features of acceleration. }
\label{tab:acc}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
 min    &     1.00 &     0.46 &      0.46 &        0.46 &     0.46 &     0.46 &     0.46 &     0.46 &     0.46 &     0.46 \\ \hline
 max    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 mean   &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 median &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 std    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 p10    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 p25    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 p50    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 p75    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline
 p90    &     0.46 &     1.00 &      1.00 &        1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 &     1.00 \\ \hline


\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{The Kruskal-Wallis test results for pair-wise trajectory features of jerk. }
\label{tab:jerk}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
 min    &      1.00 &      0.46 &       0.46 &         0.46 &      0.46 &      0.46 &      0.46 &      0.46 &      0.46 &      0.46 \\ \hline
 max    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 mean   &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 median &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 std    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 p10    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 p25    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 p50    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 p75    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline
 p90    &      0.46 &      1.00 &       1.00 &         1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 &      1.00 \\ \hline


\end{tabular}
\end{table}



\begin{table}[h]
\centering
\caption{The Kruskal-Wallis test results for pair-wise trajectory features of bearing. }
\label{tab:bearing}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
min    &         1.00 &         0.12 &          0.12 &            0.12 &         0.12 &         0.12 &         0.12 &         0.12 &         0.12 &         0.12 \\ \hline
max    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
mean   &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
median &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
std    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
p10    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
p25    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
p50    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
p75    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline
p90    &         0.12 &         1.00 &          1.00 &            1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 &         1.00 \\ \hline

\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{The Kruskal-Wallis test results for pair-wise trajectory features of bearing rate  }
\label{tab:brate}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
\textbf{ min}    &       1.00 &       0.03 &        0.03 &          0.03 &       0.03 &       0.03 &       0.03 &       0.03 &       0.03 &       0.03 \\ \hline
 max    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 mean   &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 median &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
std    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 p10    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 p25    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 p50    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 p75    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline
 p90    &       0.03 &       1.00 &        1.00 &          1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 &       1.00 \\ \hline

\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{The Kruskal-Wallis test results for pair-wise trajectory features of the rate of the bearing rate  }
\label{tab:brate2}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
                        & \textbf{min} & \textbf{max} & \textbf{mean} & \textbf{median} & \textbf{std} & \textbf{p10} & \textbf{p25} & \textbf{p50} & \textbf{p75} & \textbf{p90} \\ \hline
 min    &        1.00 &        0.35 &         0.35 &           0.35 &        0.35 &        0.35 &        0.35 &        0.35 &        0.35 &        0.35 \\ \hline
 max    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 mean   &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 median &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 std    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 p10    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 p25    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 p50    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 p75    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline
 p90    &        0.35 &        1.00 &         1.00 &           1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 &        1.00 \\ \hline

\end{tabular}
\end{table}



==> reports/report_001.tex <==
\section{report}
\subsection*{objective}ss
\subsection*{Date}Mar 31,2018
\subsection*{Dataset}
\subsection*{Method}
\subsection*{results}

==> reports/similarity.tex <==
\section{Similarity }
\subsection{Edit Distance}The Minimum Edit Distance or Levenshtein Dinstance

 \url{https://www.python-course.eu/levenshtein_distance.php}
\subsection{EDR}\cite{Chen:2004:MLE:1316689.1316758}
\subsection{Longest common sub-sequence (LCSS)}\cite{Toohey:2015:TSM:2782759.2782767}
\subsection{Cats}
\subsection{EDWp}
\subsection{UMS}
\subsection{MSM}
\subsection{TWED}\cite{marteau2009time} \cite{Chen:2004:MLE:1316689.1316758}
\subsection{Dynamic Time Wraping (DTW)}\cite{Toohey:2015:TSM:2782759.2782767}
\url{http://alexminnaar.com/time-series-classification-and-clustering-with-python.html}
 
 is quadratic in the length of the time series used
 
 distortion in the time axis
 
 speed up DTW using locality assumption
 $T_1=(t_1^1,t_2^1,...,t_n^1)$
 $T_2=(t_1^2,t_2^2,...,t_n^2)$
 
 $W_{(i,j)}=haversine(p_i,p_j)$
 γ(i,j)=d(qi,cj)+min(γ(i−1,j−1),γ(i−1,j),γ(i,j−1)) . 
 
 $\lambda_{(i,j)}=haversine(T^i,T^j)+min(\lambda_{(i-1,j-1)},\lambda_{(i-1,j)},\lambda_{(i,j-1)})$
 
 the LB Keogh lower bound of dynamic time warping
 
\subsection{Edit Distance (ED)}\cite{Toohey:2015:TSM:2782759.2782767}\cite{Chen:2004:MLE:1316689.1316758}
\subsection{Fŕechet Distance}\cite{Toohey:2015:TSM:2782759.2782767}
\subsection{shapelet}\cite{refregier2003shapelets}
\subsection{trajectory annotation}\cite{moosavi2017annotation}
\section{noise}
\subsection{ONF-TRRS}\cite{riyadh2017research}
\subsection{Extract stops}\cite{xiang2016extracting}

\section{segmentation}
\subsection{Transition based methods}\cite{zheng2008understanding}
\subsection{clustering based methods}\cite{lee2007trajectory}
\subsection{time based methods}\cite{stenneth2011transportation}
\subsection{distance based methods}\cite{liao2006location}
\subsection{window based methods}\cite{miluzzo2008sensing}
\subsection{AIS}\cite{de2016improving}
\subsection{GRASP-UTS}\cite{soares2015grasp}\cite{juniorsemi}
\section{Privacy}
\subsection{Attacks}Location Attack, Location Sequence Attack, Visit Attack, Frequent Location and Sequence Attack, Frequency Attack, Home and Work Attack\cite{pellungrini2017fast}\cite{pratesi2017privacy}\cite{liu2008survey}

